"John is 50 years old, can his son be 65?" Evaluating NLP Models' Understanding of Feasibility

In current NLP research, large-scale language models and their abilities are widely being discussed. Some recent works have also found notable failures of these models. Often these failure examples involve complex reasoning abilities. This work focuses on a simple commonsense ability, reasoning about when an action (or its effect) is feasible. To this end, we introduce FeasibilityQA, a question-answering dataset involving binary classification (BCQ) and multi-choice multi-correct questions (MCQ) that test understanding of feasibility. We show that even state-of-the-art models such as GPT-3, GPT-2, and T5 struggle to answer the feasibility questions correctly. Specifically, on MCQ and BCQ questions, GPT-3 achieves an accuracy of just (19%, 62%) and (25%, 64%) in zero-shot and few-shot settings, respectively. We also evaluate models by providing relevant knowledge statements required to answer the question. We find that the additional knowledge leads to a 7% gain in performance, but the overall performance still remains low. These results make one wonder how much commonsense knowledge about action feasibility is encoded in state-of-the-art models and how well they can reason about it.

==> Tables/binary_classification.tex <==
\begin{table*}[t!]
\small
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}p{0.4\linewidth}>{\RaggedRight}p{0.35\linewidth}>{\RaggedRight}p{0.15\linewidth}@{}}
    \toprule
        \textbf{Premise} &
        \textbf{Hypothesis} &
        \textbf{Label} 
        \\
    \midrule
    \multirow{2}{\linewidth}
          {Sam gave 50 dollars to the shopkeeper to buy a book. The shopkeeper returned some money}
          & 
          The price of the book could be 55 dollars.	& 
          False \ding{51}\\
          
          & 
          The price of the book could be 45 dollars.	& 
          True \ding{55}\\
          
          \\
     \multirow{2}{\linewidth}
          {Sam gave 50 dollars to the shopkeeper to buy a book. The shopkeeper returned some money}
          & 
          The price of the book could be 55 dollars.	& 
          False \ding{51}\\
          & 
          The price of the book could be 45 dollars.	& 
          True \ding{55}\\
    
       
    \bottomrule

    \end{tabular}
    }
    \caption{
    Illustrative examples of binary classification task in Feasibility-QA. 
    }
    \label{tab:binary_classification_examples}
\end{table*}

==> Tables/gpt_2_results.tex <==
\begin{table}[h!]
\begin{tabular}{lrr|rr}
\hline
\textbf{} & \multicolumn{2}{c|}{\textbf{BCQ}}                  & \multicolumn{2}{c}{\textbf{MCQ}}                  \\ \hline
          & \multicolumn{1}{l}{w/o K} & \multicolumn{1}{l|}{K} & \multicolumn{1}{l}{w/o K} & \multicolumn{1}{l}{K} \\ \hline
Zero Shot & 2.4                       & 0                      & 0.19                      & 0.45                  \\
One Shot  & 50                        & 50                     & 0.58                      & 1.69                  \\
Few Shot  & 50                        & 50                     & 0.97                      & 0.39                  \\ \hline
\end{tabular}

\caption{
   Accuracy of GPT-2 on BCQ and MCQ setting. The performance is $\approx$ 0\% in MCQ and 50\% in BCQ setting.
    }
    
\label{tab:gpt2_results}

\end{table}

==> Tables/mcq.tex <==
\begin{table*}[t!]
\small
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}p{0.4\linewidth}>{\RaggedRight}p{0.35\linewidth}>{\RaggedRight}p{0.15\linewidth}@{}}
    \toprule
        \textbf{Premise} &
        \textbf{Question/ Hypothesis} &
        \textbf{Options} 
        \\
    \midrule
       Sam gave 50 dollars to the shopkeeper to buy a book. The shopkeeper returned some money
      & 
      The price of the book could be 55 dollars.\newline The price of the book could be 40 dollars	& 
          False \ding{55} \newline True \ding{51}
      \\\\
      Sam gave 50 dollars to the shopkeeper to buy a book. The shopkeeper returned some money
      & 
      What could be the price of the book?
      & 
       55, \textbf{45}, \newline  \textbf{37}, None\\

       
    \bottomrule

    \end{tabular}
    }
    \caption{
    Illustrative examples of Binary Classification and Multi-correct MCQ task in Feasibility-QA. Correct answers are in bold.
    }
    \label{tab:mcq_exmples}
\end{table*}

==> Tables/mcq2.tex <==
\begin{table}[]
\resizebox{\linewidth}{!}{
\begin{tabular}{lll}
\hline
\multicolumn{3}{c}{\textbf{Premise}}                                                                                                                   \\ \hline
\multicolumn{3}{l}{\begin{tabular}[c]{@{}l@{}}Sam gave 50 dollars to the shopkeeper to buy a book. \\ The shopkeeper returned some money\end{tabular}} \\ \hline
\multicolumn{3}{c}{\textbf{Question}}                                                                                                                  \\ \hline
\multicolumn{3}{l}{\begin{tabular}[c]{@{}l@{}}The price of the book could be 55 dollars.\\ The price of the book could be 40 dollars.\end{tabular}}    \\
\multicolumn{3}{l}{What could be the price of the book?}                                                                                               \\ \hline
\multicolumn{3}{c}{\textbf{Options}}                                                                                                                   \\ \hline
\multicolumn{1}{l|}{False \ding{55} }                          & \multicolumn{1}{l|}{True  \ding{51}  }                          & 55,  \textbf{45},  \textbf{37},  None                          \\ \hline
\end{tabular}
}
\caption{
   Illustrative examples of Binary Classification and Multi-correct MCQ task in Feasibility-QA. Correct answers are in bold. 
    }
    
\label{tab:combined_examples}
\end{table}


==> Tables/mcq_results.tex <==
\begin{table}[]
\begin{tabular}{lrr}
\hline
\textbf{} & \multicolumn{1}{l}{Without  Knowledge} & \multicolumn{1}{l}{With  Knowledge} \\ \hline
Zero      & 0.19                                   & 0.25                                \\
One       & 0.209                                  & 0.24                                \\
Few       & 0.259                                  & 0.37                                \\ \hline
\end{tabular}

\caption{
   Accuracy of GPT-3 on MCQ task of FeasibilityQA Dataset in zero-shot, one-shot and few-shot settings.
    }
    
\label{tab:mcq_results}
\end{table}

==> Tables/t5_results.tex <==
\begin{table}[h!]
\begin{tabular}{lrr|rr}
\hline
\textbf{} & \multicolumn{2}{c|}{\textbf{BCQ}}                  & \multicolumn{2}{c}{\textbf{MCQ}}                  \\ \hline
          & \multicolumn{1}{l}{w/o K} & \multicolumn{1}{l|}{K} & \multicolumn{1}{l}{w/o K} & \multicolumn{1}{l}{K} \\ \hline
Zero Shot & 50.55                     & 50.64                  & 0.13                      & 0.39                  \\
One Shot  & 50.61                     & 50.33                  & 0.45                      & 0.58                  \\
Few Shot  & 49.81                     & 49.87                  & 0.84                      & 1.10                  \\ \hline
\end{tabular}

\caption{
   Accuracy of T-5 on BCQ and MCQ setting. Similar to GPT-2, the performance is $\approx$ 0\% in MCQ and 50\% in BCQ setting.
    }
    
\label{tab:t5_results}
% \vspace{-0.5cm}
\end{table}
